Interactive Control over Temporal Consistency while Stylizing Video Streams

Image stylization has seen significant advancement and widespread interest over the years, leading to the development of a multitude of techniques. Extending these stylization techniques, such as Neural Style Transfer (NST), to videos is often achieved by applying them on a per-frame basis. However, per-frame stylization usually lacks temporal consistency, expressed by undesirable flickering artifacts. Most of the existing approaches for enforcing temporal consistency suffer from one or more of the following drawbacks: They (1) are only suitable for a limited range of techniques, (2) do not support online processing as they require the complete video as input, (3) cannot provide consistency for the task of stylization, or (4) do not provide interactive consistency control. Domain-agnostic techniques for temporal consistency aim to eradicate flickering completely but typically disregard aesthetic aspects. For stylization tasks, however, consistency control is an essential requirement as a certain amount of flickering adds to the artistic look and feel. Moreover, making this control interactive is paramount from a usability perspective. To achieve the above requirements, we propose an approach that stylizes video streams in real-time at full HD resolutions while providing interactive consistency control. We develop a lite optical-flow network that operates at 80 FPS on desktop systems with sufficient accuracy. Further, we employ an adaptive combination of local and global consistency features and enable interactive selection between them. Objective and subjective evaluations demonstrate that our method is superior to state-of-the-art video consistency approaches.

==> graphics/evaluation/compare_consistency_colorization.tex <==
	\begin{subfigure}{0.240000\linewidth}
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/original/DAVIS-gray/goat/00016.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/original/DAVIS-gray/goat/00017.jpg}  
		\caption{Original}
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/processed/ECCV16_colorization/DAVIS-gray/goat/00016.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/processed/ECCV16_colorization/DAVIS-gray/goat/00017.jpg}  
		\caption{Processed, inconsistent}
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/lai/ECCV16_colorization/DAVIS-gray/goat/00016.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/lai/ECCV16_colorization/DAVIS-gray/goat/00017.jpg}  
		\caption{Lai \cite{LearningVideoConsistency}}
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/iospwc-my-light4dec-sepref-prune040-fp8extra--singlescale2nd/ECCV16_colorization/DAVIS-gray/goat/000016.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/iospwc-my-light4dec-sepref-prune040-fp8extra--singlescale2nd/ECCV16_colorization/DAVIS-gray/goat/000017.jpg}  
		\caption{Ours, mobile-optimized}
	\end{subfigure}


==> graphics/evaluation/compare_consistency_general.tex <==
	\begin{subfigure}{0.240000\linewidth}
		\adjincludegraphics[Clip={0.3\width} {0} {0} {0},width=\linewidth]{graphics/4evaluation/consistency/original/DAVIS-gray/goat/00016.jpg} \\ 
		\adjincludegraphics[Clip={0.3\width} {0} {0} {0},width=\linewidth]{graphics/4evaluation/consistency/original/DAVIS-gray/goat/00017.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/original/DAVIS/mbike-trick/00026.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/original/DAVIS/mbike-trick/00027.jpg}  
		\caption{Original}
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\adjincludegraphics[Clip={0.3\width} {0} {0} {0},width=\linewidth]{graphics/4evaluation/consistency/processed/ECCV16_colorization/DAVIS-gray/goat/00016.jpg} \\ 
		\adjincludegraphics[Clip={0.3\width} {0} {0} {0},width=\linewidth]{graphics/4evaluation/consistency/processed/ECCV16_colorization/DAVIS-gray/goat/00017.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/processed/IntrinsicDecomposition/reflectance/DAVIS/mbike-trick/00026.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/processed/IntrinsicDecomposition/reflectance/DAVIS/mbike-trick/00027.jpg}  
		\caption{Processed, inconsistent}
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\adjincludegraphics[Clip={0.3\width} {0} {0} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/lai/ECCV16_colorization/DAVIS-gray/goat/00016.jpg} \\ 
		\adjincludegraphics[Clip={0.3\width} {0} {0} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/lai/ECCV16_colorization/DAVIS-gray/goat/00017.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/lai/IntrinsicDecomposition/reflectance/DAVIS/mbike-trick/00026.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/lai/IntrinsicDecomposition/reflectance/DAVIS/mbike-trick/00027.jpg}  
		\caption{Lai \cite{LearningVideoConsistency}}
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\adjincludegraphics[Clip={0.3\width} {0} {0} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/iospwc-my-light4dec-sepref-prune040-fp8extra--singlescale2nd/ECCV16_colorization/DAVIS-gray/goat/000016.jpg} \\ 
		\adjincludegraphics[Clip={0.3\width} {0} {0} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/iospwc-my-light4dec-sepref-prune040-fp8extra--singlescale2nd/ECCV16_colorization/DAVIS-gray/goat/000017.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/iospwc-my-light4dec-sepref-prune040-fp8extra--singlescale2nd/IntrinsicDecomposition/reflectance/DAVIS/mbike-trick/000026.jpg} \\ 
		\adjincludegraphics[Clip={0} {0} {0.3\width} {0},width=\linewidth]{graphics/4evaluation/consistency/stabilized/iospwc-my-light4dec-sepref-prune040-fp8extra--singlescale2nd/IntrinsicDecomposition/reflectance/DAVIS/mbike-trick/000027.jpg}  
		\caption{Ours, mobile-optimized}
	\end{subfigure}


==> graphics/evaluation/compare_consistency_nst.tex.tex <==
	\begin{subfigure}{0.240000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/consistency/original/dm/1-woman-dancing-2873755/000010.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/consistency/original/2-lotus-dancing-in-the-wind-854695/000010.jpg}  
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/consistency/processed/dm_nst/nst_mosaic/dm/1-woman-dancing-2873755/000010.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/consistency/processed/dm_nst/nst_udnie/2-lotus-dancing-in-the-wind-854695/000010.jpg}  
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/consistency/stabilized/lai/dm_nst/nst_mosaic/dm/1-woman-dancing-2873755/000010.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/consistency/stabilized/lai/dm_nst/nst_udnie/2-lotus-dancing-in-the-wind-854695/000010.jpg}  
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/consistency/stabilized/iospwc-my-light4dec-sepref-prune040--singlescale2nd/dm_nst/nst_mosaic/dm/1-woman-dancing-2873755/000010.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/consistency/stabilized/iospwc-my-light4dec-sepref-prune040--singlescale2nd/dm_nst/nst_udnie/2-lotus-dancing-in-the-wind-854695/000010.jpg}  
	\end{subfigure}


==> graphics/evaluation/compare_epe_sintelfinal_ablation.tex <==
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00565_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00650_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00246_flow_gt.jpg}  
		\caption{Ground-truth}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{PWCNet (5dense)}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{5light}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{4light-sepref}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{4light-sepref-prune40}
	\end{subfigure}


==> graphics/evaluation/compare_epe_sintelfinal_ablationextra.tex <==
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{5light}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-seplight-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-seplight-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-seplight-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{5light-5sep}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-part2seplight-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-part2seplight-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-part2seplight-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{5light-2sep}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta75-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta75-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta75-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{5light-c75}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta50-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta50-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta50-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{5light-c50}
	\end{subfigure}


==> graphics/evaluation/compare_epe_sintelfinal_coarse.tex <==
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00565_img_overlayed.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00203_img_overlayed.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00650_img_overlayed.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00246_img_overlayed.jpg}  
		\caption{Frame Overlay}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00565_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00203_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00650_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00246_flow_gt.jpg}  
		\caption{Ground-truth}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00203_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/raft-sintel/vis_00246_epe.jpg}  
		\caption{RAFT \cite{RAFT}}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-ft-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-ft-sintel/vis_00203_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-ft-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-ft-sintel/vis_00246_epe.jpg}  
		\caption{PWC-Net \cite{PWCNet}}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-light4dec-sepref-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-light4dec-sepref-chairs-things-sintel/vis_00203_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-light4dec-sepref-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-light4dec-sepref-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{Ours}
	\end{subfigure}


==> graphics/evaluation/compare_epe_sintelfinal_coarsemobile.tex <==
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00565_img_overlayed.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00203_img_overlayed.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00650_img_overlayed.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00246_img_overlayed.jpg}  
		\caption{Frame Overlay}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00565_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00203_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00650_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00246_flow_gt.jpg}  
		\caption{Ground-truth}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00203_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00246_epe.jpg}  
		\caption{iOS Flow \cite{iOSFlow}}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00203_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{PWC-Net \cite{PWCNet}}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00565_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00203_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00650_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00246_epe.jpg}  
		\caption{Ours}
	\end{subfigure}


==> graphics/evaluation/compare_flow_davis_coarsemobile.tex <==
	\begin{subfigure}{0.240000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iosflow-veryhigh/vis_00159_img_overlayed.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iosflow-veryhigh/vis_00005_img_overlayed.jpg}  
		%\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iosflow-veryhigh/vis_00266_img_overlayed.jpg} \\ 
		%\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iosflow-veryhigh/vis_00073_img_overlayed.jpg}  
		\caption{Frame Overlay}
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00159_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00005_flow_fwd.jpg}  
		%\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00266_flow_fwd.jpg} \\ 
		%\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00073_flow_fwd.jpg}  
		\caption{PWC-Net \cite{PWCNet}}
	\end{subfigure}
	\begin{subfigure}{0.240000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00159_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00005_flow_fwd.jpg}  
		%\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00266_flow_fwd.jpg} \\ 
		%\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00073_flow_fwd.jpg}  
		\caption{Ours}
	\end{subfigure}
    \begin{subfigure}{0.240000\linewidth}
    	\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iosflow-veryhigh/vis_00159_flow_fwd.jpg} \\ 
    	\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iosflow-veryhigh/vis_00005_flow_fwd.jpg} 
    	%\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iosflow-veryhigh/vis_00266_flow_fwd.jpg} \\ 
    	%\includegraphics[width=\linewidth]{graphics/evaluation/davisvis/iosflow-veryhigh/vis_00073_flow_fwd.jpg}  
    	\caption{iOS Flow \cite{iOSFlow}}
    \end{subfigure}


==> graphics/evaluation/compare_flow_sintelfinal_ablation.tex <==
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00565_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00650_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00246_flow_gt.jpg}  
		\caption{Ground-truth}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{PWCNet (5dense)}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{5light}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{4light-sepref}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{4light-sepref-prune40}
	\end{subfigure}


==> graphics/evaluation/compare_flow_sintelfinal_ablationextra.tex <==
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\  
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{5light}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-seplight-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-seplight-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-seplight-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{5light-5sep}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-part2seplight-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-part2seplight-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-part2seplight-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{5light-2sep}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta75-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta75-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta75-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{5light-c75}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta50-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta50-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-lighta50-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{5light-c50}
	\end{subfigure}


==> graphics/evaluation/compare_flow_sintelfinal_coarsemobile.tex <==
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00565_img_overlayed.jpg} \\ 
		%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00203_img_overlayed.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00650_img_overlayed.jpg}  
		%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00246_img_overlayed.jpg}  
		\caption{Frame Overlay}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00565_flow_gt.jpg} \\ 
		%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00203_flow_gt.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00650_flow_gt.jpg}  
		%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00246_flow_gt.jpg}  
		\caption{Ground-truth}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00203_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg}  
		%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{PWC-Net \cite{PWCNet}}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00565_flow_fwd.jpg} \\ 
		%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00203_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00650_flow_fwd.jpg}  
		%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iospwc-my-light4dec-sepref-prune040-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{Ours}
	\end{subfigure}
	\begin{subfigure}{0.192000\linewidth}
	\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00565_flow_fwd.jpg} \\ 
	%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00203_flow_fwd.jpg} \\ 
	\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00650_flow_fwd.jpg} 
	%\includegraphics[width=\linewidth]{graphics/evaluation/sintelfinal/iosflow-veryhigh/vis_00246_flow_fwd.jpg}  
	\caption{iOS Flow \cite{iOSFlow}}
    \end{subfigure}


==> graphics/evaluation/compare_flow_sintelfinal_desktopvsmobile1.tex <==
	\begin{subfigure}{0.320000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-dense-chairs-things-sintel/vis_00203_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-dense-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{Desktop}
	\end{subfigure}
	\begin{subfigure}{0.320000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00203_ref_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00246_ref_epe.jpg}  
		\caption{Ref EPE}
	\end{subfigure}
	\begin{subfigure}{0.320000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00203_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{Mobile}
	\end{subfigure}


==> graphics/evaluation/compare_flow_sintelfinal_desktopvsmobile2.tex <==
	\begin{subfigure}{0.320000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-light4dec-sepref-chairs-things-sintel/vis_00203_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-light4dec-sepref-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{Desktop}
	\end{subfigure}
	\begin{subfigure}{0.320000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00203_ref_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00246_ref_epe.jpg}  
		\caption{Ref EPE}
	\end{subfigure}
	\begin{subfigure}{0.320000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00203_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-light4dec-sepref-fp8extra-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{Mobile}
	\end{subfigure}


==> graphics/evaluation/compare_flow_sintelfinal_desktopvsmobile3.tex <==
	\begin{subfigure}{0.320000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-dense-chairs-things-sintel/vis_00203_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/pwcnet-my-dense-chairs-things-sintel/vis_00246_flow_fwd.jpg}  
		\caption{Desktop}
	\end{subfigure}
	\begin{subfigure}{0.320000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel-upconvnopad/vis_00203_ref_epe.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel-upconvnopad/vis_00246_ref_epe.jpg}  
		\caption{Ref EPE}
	\end{subfigure}
	\begin{subfigure}{0.320000\linewidth}
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel-upconvnopad/vis_00203_flow_fwd.jpg} \\ 
		\includegraphics[width=\linewidth]{graphics/4evaluation/sintelfinal/iospwc-my-dense-fp8extra-chairs-things-sintel-upconvnopad/vis_00246_flow_fwd.jpg}  
		\caption{Mobile}
	\end{subfigure}


==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\etal{\textit{et~al}\onedot~}
\def\eg{e.g\onedot, } 
\def\ie{i.e\onedot, } 
\def\cf{cf\onedot} 
\def\wrt{w.r.t\onedot}
\def\etc{etc\onedot} 
\def\vs{vs\onedot}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text editing macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\clap#1{\hbox to 0pt{\hss #1\hss}}%
\def\initials#1{\protect\clap{\smash{\raisebox{1.4ex}{\tiny{\textsf{\textit{#1}}}}}}}%
%
\makeatletter
\newcommand{\EDIT}[4][]{\protect\@ifundefined{hidecomments}{%
  \strut{\color{#3}{\hspace{0pt}\initials{#2}\protect\sout{#1}{~#4}}}%
  }{}}
\newcommand{\NOTEboxed}[3]{\protect\@ifundefined{hidecomments}{%
  {\begin{center}\fbox{\parbox{0.97\linewidth}{\protect\EDIT{#1}{#2}{#3}}}\end{center}}
  }{}}
\makeatletter
\newcommand{\DefAuthor}[2] % initials, color
{%
  \expandafter\newcommand\csname #1edit\endcsname[2][]{\protect\EDIT[##1]{#1}{#2}{##2}}
  \expandafter\newcommand\csname #1\endcsname[1]{\protect\csname #1edit\endcsname{[##1]}}
  \expandafter\newcommand\csname #1boxed\endcsname[1]{\NOTEboxed{#1}{#2}{##1}}
}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% math macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% number sets
\def \NN {{\mathbb N}}
\def \QQ {{\mathbb Q}}
\def \ZZ {{\mathbb Z}}
\def \RR {{\mathbb R}}
\def \CC {{\mathbb C}}

% points, vectors, matrices
\newcommand{\bv}[1]{{\ensuremath{\vec{\boldsymbol #1}}}}
\newcommand{\nv}[1]{{\ensuremath{\hat{\boldsymbol #1}}}}
\newcommand{\bp}[1]{{\ensuremath{\boldsymbol #1}}}
\newcommand{\Vecc}[2]{{\renewcommand{\arraystretch}{0.8}%
    \begin{pmatrix}#1\\#2\end{pmatrix}}}
\newcommand{\Veccc}[3]{{\renewcommand{\arraystretch}{0.8}%
    \begin{pmatrix}#1\\#2\\#3\end{pmatrix}}}
\newcommand{\Vecccc}[4]{{\renewcommand{\arraystretch}{0.8}%
    \begin{pmatrix}#1\\#2\\#3\\#4\end{pmatrix}}}
\newcommand{\hVecc}[2]{{\left( #1, #2\right)}}
\newcommand{\hVeccc}[3]{{\left( #1, #2, #3\right)}}
\newcommand{\hVecccc}[4]{{\left( #1, #2, #3, #4\right)}}
\newcommand{\abs}[1]{ \left| #1 \right| }
\newcommand{\norm}[1]{ \left\| #1 \right\| }
\newcommand{\pnorm}[2]{ \left\| #1 \right\|_{#2} }
\newcommand{\cross}[2]{{#1\times#2}}
\newcommand{\dotb}[2]{{\left(#1\cdot#2\right)}}
\newcommand{\dota}[2]{ \left\langle \; {#1} \mid {#2} \; \right\rangle }

%% partial differentials
\newcommand{\pd}[2]{\frac{d #1}{d #2} }
\newcommand{\PD}[2]{\frac{\partial #1}{\partial #2} }
\newcommand{\PDDq}[2]{\frac{\partial^2 #1}{\partial #2^2} }
\newcommand{\PDD}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3} }

% operators
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\clip}{clip}
%\DeclareMathOperator*{\rank}{rank}
%\DeclareMathOperator*{\sgn} {sgn}
%\DeclareMathOperator*{\spur}{spur}
%\DeclareMathOperator*{\supp}{supp}
\def \andop {\ensuremath{\wedge}}
\def \orop  {\ensuremath{\vee}}
\def \exorop  {\ensuremath{\widehat{\;}}}
\def \implop  {\ensuremath{\rightarrow}}
\def \equivop  {\ensuremath{\leftrightarrow}}
\newcommand{\negop}[1]{\ensuremath{\neg #1}}

% other
\def \to {,\ldots ,}
